EasyPPO: Stabilizing the Critic Is Key

A key strength of Proximal Policy Optimization (PPO) is its learned critic, which uses historical trajectories collected during reinforcement learning to estimate expected returns and reduce policy-gradient variance. However, we find that the critic is also a major source of instability in reinforcement learning for large language models (LLMs). We identify two critic failure modes that destabilize PPO. First, filtering truncated rollouts from both actor and critic shifts the policy objective to reward conditioned on completion, allowing truncation to increase even as conditional reward improves. Second, heterogeneous return noise can cause high-variance prompts to dominate critic updates in finite batches. We introduce EasyPPO to address these failures. Actor-only overlong filtering trains the critic on returns from both completed and truncated rollouts. Noise-normalized critic regression weights each prompt's critic loss by the inverse standard deviation of its sampled returns, balancing noise contributions across prompts. Moderately smaller critic mini-batches confine outlier influence to fewer rollouts during gradient clipping. Across continuous-reward coding on FrontierCS, binary-reward mathematical reasoning on AIME24, and multi-turn search on Search-R1, EasyPPO remains stable throughout the full training horizon and consistently outperforms vanilla PPO, VAPO, and HL-Gauss PPO. Its best validation scores show relative gains of 14.89%, 2.28%, and 9.47% over PPO, respectively.

==> packages.tex <==
%%==================== Math ====================
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools}                % 必须在 amsmath 之后
\RequirePackage{bm}                       % commands.tex 的 \vzero 等依赖
\RequirePackage{mathpazo}

%%==================== 排版 / 字体 ====================
\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}
\RequirePackage{tocloft}
% Headings and author metadata use the same Palatino family as the body.

%%==================== 颜色 ====================
\RequirePackage{xcolor}
\RequirePackage{colortbl}
%% ---- Google GM2 palette (single source; see CLAUDE.md "Color palette") ----
\definecolor{gblue}{HTML}{1A73E8}     % blue 600
\definecolor{gred}{HTML}{D93025}      % red 600
\definecolor{gyellow}{HTML}{E37400}   % yellow 900, the only Google yellow at 3:1 on white
\definecolor{ggreen}{HTML}{1E8E3E}    % green 600
\definecolor{gpurple}{HTML}{9334E6}   % purple 600
\definecolor{ggrey}{HTML}{5F6368}     % grey 700
\colorlet{linkcol}{gblue}

%%==================== 图与排版插入 ====================
\RequirePackage{graphicx}
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz}                     % \circled 依赖

%%==================== Caption ====================
\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption}               % 必须在 caption 之后

%%==================== 表格 ====================
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{makecell}

%%==================== 布局 ====================
\RequirePackage{geometry}
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}

%%==================== 工具 ====================
\RequirePackage{verbatim}
\RequirePackage{pifont}

%%==================== 算法 ====================
\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}
\RequirePackage{minted}                   % 需 -shell-escape

%%==================== Bib ====================
\RequirePackage[numbers,sort&compress]{natbib}

%%==================== Hyperref（必须最后加载）====================
\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref} % 必须在 hyperref 之后

